Redshift evolution and covariances for joint lensing and clustering studies with DESI Y1

Galaxy-galaxy lensing (GGL) and clustering measurements from the Dark Energy Spectroscopic Instrument Year 1 (DESI Y1) dataset promise to yield unprecedented combined-probe tests of cosmology and the galaxy-halo connection. In such analyses, it is essential to identify and characterise all relevant statistical and systematic errors. In this paper, we forecast the covariances of DESI Y1 GGL+clustering measurements and characterise the systematic bias due to redshift evolution in the lens samples. Focusing on the projected clustering and galaxy-galaxy lensing correlations, we compute a Gaussian analytical covariance, using a suite of N-body and log-normal simulations to characterise the effect of the survey footprint. Using the DESI One Percent Survey data, we measure the evolution of galaxy bias parameters for the DESI Luminous Red Galaxy (LRG) and Bright Galaxy Survey (BGS) samples. We find mild evolution in the LRGs in 0.4 < z < 0.8, subdominant compared to the expected statistical errors. For BGS, we find less evolution effects for brighter absolute magnitude cuts, at the cost of reduced sample size. We find that with a fiducial redshift bin width delta z = 0.1, evolution effects on GGL is negligible across all scales, all fiducial selection cuts, all fiducial redshift bins, given DESI Y1 sample size. Galaxy clustering is more sensitive to evolution due to the bias squared scaling. Nevertheless the redshift evolution effect is insignificant for clustering above the 1-halo scale of 0.1Mpc/h. For studies that wish to reliably access smaller scales, additional treatment of redshift evolution is likely needed. This study serves as a reference for GGL and clustering studies using the DESI Y1 sample

==> oldplots/oldtext.tex <==

% Using dark emulator and the interpolated HOD, we can calculate the DS prediction as a function of redshift. 
% \begin{figure*}
%     \hspace{-0.7cm}
%     \includegraphics[width=0.8\textwidth]{plot_ds_lrg_newhodfit_proposal_0.4_0.6_0.8.pdf}
%     \vspace{-0.3cm}
%     \caption{The DS spread for the LRGs in the fiducial bins. The dark grey lines show the DS prediction assuming a single redshift at $z = 0.5$ and $z = 0.7$. }
%     \label{fig:lrg_ds}
% \end{figure*}

% \begin{figure}
%     \hspace{-0.7cm}
%     \includegraphics[width=0.5\textwidth]{plot_dserr_lrg_newhodfit_proposal_0.4_0.6_0.8.pdf}
%     \vspace{-0.3cm}
%     \caption{The relative DS error for the LRGs in the fiducial bins. The solid lines show the error induced by fiducial redshift binning assuming a model calculated at single redshifts fixed at simulation snapshots $z = 0.5$ and $z = 0.7$. The dashed lines show the error against a theory model calculated at the mean redshift of the sample. }
%     \label{fig:lrg_dserr}
% \end{figure}

% For the theory-based models evaluated at mean redshifts, the typical error is below 0.2$\%$. For the simulation-based models evaluated at snapshot redshifts, the lower redshift bin displays larger errors at just above 0.5$\%$. These errors are below the error budget. 

% \subsection{BGS}
% We first test the fiducial bins for the BGS sample with $M_r^{abs}<-19$ cut. 
% \begin{figure*}
%     \hspace{-0.7cm}
%     \includegraphics[width=0.9\textwidth]{plot_ds_bgs_proposal_0.1_0.2_0.3_0.4_magcut-19.pdf}
%     \vspace{-0.3cm}
%     \caption{The DS spread for the BGS in the fiducial bins, assuming a magnitude limited sample $M_r^{abs}<-19$. The dark grey lines show the DS prediction assuming a single redshift at $z = 0.2$ $z = 0.3$ and $z = 0.4$. }
%     \label{fig:bgs_ds}
% \end{figure*}

% \begin{figure*}
%     \hspace{-0.7cm}
%     \includegraphics[width=0.8\textwidth]{plot_dserr_bgs_proposal_0.1_0.2_0.3_0.4_magcut-19.pdf}
%     \vspace{-0.3cm}
%     \caption{The relative DS error for the BGS in the fiducial bins, assuming a magnitude limited sample $M_r^{abs}<-19$. The solid lines show the error induced by fiducial redshift binning assuming a model calculated at single redshifts fixed at simulation snapshots $z = 0.2$ $z = 0.3$ and $z = 0.4$. The dashed lines show the error against a theory model calculated at the mean redshift of the sample. }
%     \label{fig:bgs_dserr}
% \end{figure*}

% The fiducial bins works well for the theory-based models, but not for the simulation-based models. We propose an alternative binning scheme centered around Abacus output redshifts for simulation-based analyses. 

% \begin{figure*}
%     \hspace{-0.7cm}
%     \includegraphics[width=0.9\textwidth]{plot_ds_bgs_proposal_0.15_0.25_0.35_0.45_magcut-19.pdf}
%     \vspace{-0.3cm}
%     \caption{The DS spread for the BGS in the alternative bins, assuming a magnitude limited sample $M_r^{abs}<-19$. The dark grey lines show the DS prediction assuming a single redshift at $z = 0.2$ $z = 0.3$ and $z = 0.4$. }
%     \label{fig:bgs_ds_alt}
% \end{figure*}

% \begin{figure*}
%     \hspace{-0.7cm}
%     \includegraphics[width=0.8\textwidth]{plot_dserr_bgs_proposal_0.15_0.25_0.35_0.45_magcut-19.pdf}
%     \vspace{-0.3cm}
%     \caption{The relative DS error for the BGS in the alternative bins, assuming a magnitude limited sample $M_r^{abs}<-19$. The solid lines show the error induced by fiducial redshift binning assuming a model calculated at single redshifts fixed at simulation snapshots $z = 0.2$ $z = 0.3$ and $z = 0.4$. The dashed lines show the error against a theory model calculated at the mean redshift of the sample. }
%     \label{fig:bgs_dserr_alt}
% \end{figure*}

% The alternative model works significantly better for simulation-based models. However, the errors are still large at over 1$\%$ in htte $0.15 < z < 0.25$ bin. This is because of the highly non-linear redshift evolution in the HOD at around $z = 0.2$. The $M_r^{abs}<-20$ sample shows significantly less evolution in the HOD, so it might be a better sample for controlling HOD systematics at the cost of losing another 30$\%$ of the sample. We test this sample below. 

% \begin{figure*}
%     \hspace{-0.7cm}
%     \includegraphics[width=0.9\textwidth]{plot_ds_bgs_proposal_0.15_0.25_0.35_0.45_magcut-20.pdf}
%     \vspace{-0.3cm}
%     \caption{The DS spread for the BGS in the alternative bins, assuming a magnitude limited sample $M_r^{abs}<-20$. The dark grey lines show the DS prediction assuming a single redshift at $z = 0.2$ $z = 0.3$ and $z = 0.4$. }
%     \label{fig:bgs_ds_alt20}
% \end{figure*}

% \begin{figure*}
%     \hspace{-0.7cm}
%     \includegraphics[width=0.8\textwidth]{plot_dserr_bgs_proposal_0.15_0.25_0.35_0.45_magcut-20.pdf}
%     \vspace{-0.3cm}
%     \caption{The relative DS error for the BGS in the alternative bins, assuming a magnitude limited sample $M_r^{abs}<-20$. The solid lines show the error induced by fiducial redshift binning assuming a model calculated at single redshifts fixed at simulation snapshots $z = 0.2$ $z = 0.3$ and $z = 0.4$. The dashed lines show the error against a theory model calculated at the mean redshift of the sample. }
%     \label{fig:bgs_dserr_alt20}
% \end{figure*}

As expected, the $M_r^{abs}<-20$ shows significantly smaller errors. 

